Towards Frequency-Based Explanation for Robust CNN

Current explanation techniques towards a transparent Convolutional Neural Network (CNN) mainly focuses on building connections between the human-understandable input features with models' prediction, overlooking an alternative representation of the input, the frequency components decomposition. In this work, we present an analysis of the connection between the distribution of frequency components in the input dataset and the reasoning process the model learns from the data. We further provide quantification analysis about the contribution of different frequency components toward the model's prediction. We show that the vulnerability of the model against tiny distortions is a result of the model is relying on the high-frequency features, the target features of the adversarial (black and white-box) attackers, to make the prediction. We further show that if the model develops stronger association between the low-frequency component with true labels, the model is more robust, which is the explanation of why adversarially trained models are more robust against tiny distortions.

==> 06_Followups.tex <==
\section{Follow-ups}
\label{sec: follow-up}
Since a robust model is trained to rely more on the low-frequency features and the adversarial attacks we have shown above tends to perturb the high-frequency features, we are considering that if the input images contain as least middle-frequency and high-frequency features as possible, then the model will be less likely to learn the high-frequency patterns since they are very limited. And if the model is not able to use the middle-frequency and high-frequency features, the adversarial attacks are not able to flip the prediction by perturbing the middle-frequency and high-frequency features since there are fewer of them. Therefore, we propose to develop a prepossessing technique that shift the distribution of the frequency spectrum in the input to ensure the energy is clustering in the low frequency range. We do not want to simply zero-out the high-frequency frequency components in the input since the model may not generalize well as mentioned by \citet{Haohan-2020}

\subsection{Characterize perturbations of the attack}
We also propose use of average Maximum Mean Discrepancies (AMMD) as metric to characterize the overall perturbations of images in frequency domain. Maximum Mean Discrepancies (MMD) is just the distance between the means of the two distributions. Matching distributions like this will match their means, though they might differ in their variance or in other ways. It is calculated as follow
For the given distribution $P$  and $Q$
\begin{equation}
\text{MMD}(P,Q) = \| \mu_P - \mu_Q \|_\mathcal{H}
\end{equation}
where $\mu_P= \int k(\cdot,x) dP(x)$ and $\mu_Q = \int k(\cdot,x) dQ(x) $ are kernel means. For this work the $P$ and $Q$ are the DCT transforms of image $x$ and $x'$. We calculate average MMD with gaussian kernel as follows
\begin{equation}
\text{AMMD}(\mathcal{F}(x),\mathcal{F}(x')) = \frac{1}{\text{N}}\sum_{\text{i}=1}^{\text{N}}\| \mu_{\mathcal{F}(x_i)} - \mu_{\mathcal{F}(x_i')} \|_\mathcal{H}
\end{equation}

\begin{table}[ht]
\begin{center}
\begin{tabular}{| c|| c| c| }
\hline
\textbf{Attack \textbackslash Measures}  & \textbf{Accuracy} & \textbf{AMMD}\\ 
\hline
\hline
 \textbf{Original model} & 34.5\% & 0 \\  
\hline
\textbf{ PGD Attack} & 0\% & .0073 \\  
\hline
 \textbf{FGSM Attack }& 12.5\% & .1385 \\
 \hline
\textbf{ CW Attack} & 0\% & 1.2924e-06 \\
 \hline
\textbf{  L-BFGS Attack }& 46\% & .0257 \\
 \hline
%  Jacobian Attack & cell8 & cell9 \\
%  \hline
\end{tabular}
\caption{VGG16 performance on perturbed some 200 test samples and corresponding MMD distance specifying average perturbation of images in frequency domain}
\label{tab:MMD}
\end{center}
\end{table}

The preliminary results of some of the attacks on CIFAR10 dataset are shown in table \ref{tab:MMD}. We believe that using AMMD metric we can get some intuition on how well an undefended model will behave on an adversarial dataset. This metric can help in designing the defense of the model
